SoK: Decoding the Super App Enigma: The Security Mechanisms, Threats, and Trade-offs in OS-alike Apps

The super app paradigm, exemplified by platforms such as WeChat and AliPay, has revolutionized the mobile app landscape by enabling third-party developers to deploy add-ons within these apps. These add-ons, known as miniapps, leverage user data hosted by the super app platforms to provide a wide range of services, such as shopping and gaming. With the rise of miniapps, super apps have transformed into "operating systems", offering encapsulated APIs to miniapp developers as well as in-app miniapp stores for users to explore and download miniapps. In this paper, we provide the first systematic study to consolidate the current state of knowledge in this field from the security perspective: the security measures, threats, and trade-offs of this paradigm. Specifically, we summarize 13 security mechanisms and 10 security threats in super app platforms, followed by a root cause analysis revealing that the security assumptions still may be violated due to issues in underlying systems, implementation of isolation, and vetting. Additionally, we also systematize open problems and trade-offs that need to be addressed by future works to help enhance the security and privacy of this new paradigm.

==> paper/03_overview.tex <==


\paragraph{Methodology} To conduct our research study, we adopt a bottom-up approach. The methodology commences with the collection of information on various super apps, including their evolution, and a thorough review of available papers and reports. Initially, the study focuses on summarising the defenses applied by super app platforms across the miniapp developing and execution by reading through the documentations and actually using or developing miniapps as real users or developers. After that, we proceed to analyze the defense mechanisms by compiling the existing research papers and reports on the security and threats of super app platforms collected from top venues and CVE databases. Based on these threats and vulnerabilities, we identify the root causes and tabularize them to create a systematic understanding as well as to motivate new problems for future studies. In the end, we identify the dilemmas and potential trade-offs on the conflict of interests between the developers, users, and the super app platforms, where future works could be carried out to address the balance between these parties.


%\AY{write a architecture of how this study is conducted. Use a bottom-up approach, first collect the super apps and papers/reports. The good: show how the miniapps evolved from old paradigms, combined with the threat model, show why they are good for security. The bad: summarize the existing reports and papers to analyze the root cause, categorize them into the table. The dilemmas/hard-to-address problems: show the messages pulled from user forum and official announcements, to address the privacy concern from users, convenience concerns from developers, and especially the malware detection concern from super apps: these are the potential problems to work on.}

\paragraph{Threat Model and Scope} This research study's threat model examines vulnerabilities within super apps and miniapps, considering potential victims and attackers. The super apps themselves are not assumed to be malicious. Potential victims include users, developers, and the super apps. Users face threats like privacy breaches, data leaks, unauthorized access, and financial fraud. Developers may experience data leakage and intellectual property theft. Super apps can also be targeted with denial-of-service or supply chain attacks. Attackers are divided into malicious users and developers. Malicious users exploit vulnerabilities to gain unauthorized access, steal data, or disrupt app functionality. Malicious developers create and distribute harmful miniapps, inject code into legitimate ones, or exploit super app vulnerabilities. The study primarily focuses on Integrated-JS-engine-based super apps, as issues in other types are similar to web and mobile security.

%The threat model of this research study focuses on the vulnerabilities that may exist within both the super apps and the miniapps, while considering the potential victims and attackers involved. It is important to note that we do not assume the super apps themselves to be malicious entities.    The potential victims in this threat model encompass three main entities: users, developers, and the super apps themselves. Users can be targeted by various threats, including privacy breaches, data leaks, unauthorized access to personal information, or financial fraud. Developers may face threats such as data leakage or intellectual property theft. Super apps, while not considered malicious, can also fall victim to attacks, such as denial-of-service attacks or supply chain attacks targeting the apps hosted on their platforms. On the other hand, the attackers in this threat model can be categorized into two primary types: malicious users and malicious developers. Malicious users may attempt to exploit vulnerabilities in the super apps or miniapps to gain unauthorized access, steal sensitive data, or disrupt the normal functioning of the apps. Malicious developers, on the other hand, may engage in activities such as creating and distributing malicious miniapps, injecting harmful code into legitimate miniapps, or exploiting vulnerabilities in the super apps to compromise user data or breach security measures.  Finally, it is important to emphasize that the research study primarily focuses on Integrated-JS-engine-based super apps, as the problems existing in other types of super apps are similar to traditional web security and mobile security. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/studioverview.pdf}
%     \caption{An overview of the methodology followed by this paper}
%     \label{fig:overview}
% \end{figure}

% \paragraph{Dataset}
% As illustrated in the figure \autoref{fig:overview}, we collected 15 sets of documentations from the super app platforms covered in this paper (note that multiple super app platforms may be owned by a same company and share same set of documentations). Besides, we collected 6 research paper published in the recent 3 years, and \AY{TODO} CVE reports collected from NVD databases related to super apps and miniapps. Meanwhile, we collected \AY{TODO} posts from developer forums of WeChat to illustrate the concerns and complaints raised from users and developers that may be subject to design dilemmas and trade-offs.
% List of papers:
% P1 H. Lu et al. Resource management risks
% P2 Y.Yang CMRF
% P3 L. Zhang, Identity Confusion
% P4 C. Wang, TaintMini
% P5 C. Wang, Hidden API
% P6 Y. Zhang, key misuse

% List of CVE reports
% CVE1
% CVE2

% List of documentations:
% DOC 1 2 3.....

% List of 




% \subsection{Problem Statement}

% However, the escalated complexity and data redistribution may introduce security and privacy concerns. More specifically, we are particularly interested in three research questions.

% \begin{packeditemize}
%     \item \paragraph{The Good: Motivation}
%     \item \paragraph{The Bad: Security and Privacy Concerns} When third-party developers can use the user data collected by the super app, privacy and security concerns arise as users may not be aware of data usage or even abuse. For instance, are the users notified on the data access from the miniprogram developers? How could the miniprograms' behaviors be fully monitored by super apps from data abuse when part of the miniprogram logic is in developers' private cloud server which is inaccessible from the super apps? Security-wise, how could the super apps ensure detection of malware and prevent them from being released? How could the security mechanisms enforced in such an OS-like app system be of similar secure level compared with traditional OS to effectively thwart attackers from exploiting the system?
%     \item \paragraph{The Ugly: Trade-offs to be Balanced}
% \end{packeditemize}

% % Moreover, witnessed by multiple reports of vulnerabilities in super apps, what factors are hindering the security of super apps, and how the competing factors and dilemmas could be addressed? 

% % Motivated by this


% % multiple frameworks there are discrepancies
% % new paradigms introduce new challenges 
% % more complex

% \subsection{Scope}

% in this paper, we mainly refer to the miniprogram paradigms, where supporting platforms themselves provide a specialized type of service to a massive amount of users, acting as an essential role for broking the user data access between developers and users to provide commercial services.



==> paper/07_discussion.tex <==
\paragraph{Everything Old is New Again}
Many of the challenges faced by super apps and mini-apps overlap with those encountered in traditional mobile apps and web apps, as depicted in \autoref{tab:threats}. For instance, phishing attacks pose a threat to both mobile apps and web apps. Similarly, hidden APIs are a well-known concern in the mobile and web domains, where attackers exploit APIs for malicious purposes. However, there are notable differences, primarily due to the integration of multiple services and functionalities within a single app. These differences can amplify security and privacy concerns. One significant distinction is the collection and distribution of sensitive information by super apps to mini-apps directly. In traditional web apps or mobile apps, the operating system or web browsers do not typically collect user information and deliver it to mini-apps.
For example, in a super app, the main app may gather personal data like financial details, location information, and other sensitive data. This data is then shared with the miniapps integrated within the super app. This integration introduces additional risks, as the responsibility for safeguarding user information extends to all miniapps and their developers. 

\paragraph{One Leak Sinks Great Ship} While super apps may implement robust security mechanisms, such as cryptographic protocols, the presence of a vulnerable component within the system can compromise the overall security posture. For example, in (T8), developers   use cryptographic protocols to protect data in transit and at rest within super apps. These protocols provide a strong layer of encryption to safeguard sensitive information. However, if the developers unintentionally or negligently hardcode cryptographic keys or other sensitive credentials within the front-end code of the mini-apps, they introduce a significant vulnerability. Once the keys are obtained, the attacker can then misuse them to compromise the security of the entire system. By recognizing and addressing the weakest links within the chain, such as proper handling of sensitive credentials, super apps and mini-apps can enhance their overall security posture and protect against potential attacks and breaches. It is crucial to adopt a holistic approach to security, focusing not only on the core security mechanisms but also on the secure development and deployment of all components within the system.

\paragraph{Authority Accompanies Responsibility} The primary responsibility for safeguarding privileges and protecting user data rests with the super app provider. It is imperative that they ensure thorough security assessments are conducted on the miniapps hosted on their platform, while also enforcing strict adherence to guidelines. However, if the super app provider fails to adequately protect the privileges granted to miniapps, it can lead to severe security and privacy risks. 
For instance, in (T3), attackers can exploit vulnerabilities within the hidden APIs to gain unauthorized access to sensitive user data or carry out malicious activities. Similarly, in (T4), attackers can abuse the cross miniapp channels to inject fake messages into other miniapps. 
To effectively mitigate these risks, it is crucial for the super app provider to prioritize security and privacy as fundamental pillars of their platform, especially when the super apps grant privileges to users or miniapps. In order to achieve this, they should establish well-defined security guidelines and ensure their strict enforcement across all miniapps within their ecosystem.

% Furthermore, the seamless nature of super apps can create potential privacy concerns. Since various services and functionalities are consolidated within a single app, the flow of data between these components may not always be transparent to the user. Users may unknowingly share their data with different mini-apps, raising questions about informed consent and control over personal information. Developers must prioritize user consent, provide clear information about data sharing practices, and offer granular controls for managing permissions and data access.

% The collection and distribution of sensitive information to mini-apps and the potential lack of transparency in data flows within the app are distinct aspects that require specific attention.

% \subsection{Redesigning the Security Model}

% \subsection{Standardizing the Framework and APIs}

% \subsection{Enhancing Malware Protection}

==> paper/cheat-classification-figure.tex <==
\begin{figure*}[t]
        \centering
        %\resizebox{\columnwidth}{!} 
        {\includegraphics[width=7in]{images/hkk_countermeasure.png}}
        \caption{\hkk{Overview of online game security countermeasures.\ZQ{This figure looks nice. The resolution of this figure isn't good. Can you please share the source of this figure? We may need to consolidate this figure with Table 1}} \hkk{got it. see the fig1.pptx . you can freely modify the file. }}
        \label{fig:game_countermeasure}
\end{figure*}



==> paper/cheat-classification-tbl.tex <==

\begin{table*}[t]
\centering
\caption{\hkk{Cheating detection methods on client-, network-, and server-side (will be re-written and polished)}}
\label{table:cheating_detection_method}

\scalebox{0.80}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
                                                              & \textbf{Method}                                                                          & \textbf{Example}                                                                                                                           & \textbf{Drawback}                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Client-side detection}}  & Signature-based                                                                          & PunkBuster                                                                                                                                 & - Only works for well-known cheats.                                                                                                                             \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Third-party security\\ solution\end{tabular}                  & Hackshield, GameGuard                                                                                                                      & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}- Occupying client's resources.\\ - Conflict with other security solution,\\ AV, or even system kernel\end{tabular}} \\ \cline{2-3}
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Game devloper's security\\ solution\end{tabular}              & Blizzard's Warden Client, TenGuard, NexonGuard                                                                                             &                                                                                                                                                                 \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & In-game trap                                                                             & Invisible NPC (Non-Player Character), dummy, or item                                                                                       & - Temporal method (trap only valid until unveiled)                                                                                                                    \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & Anti-debugger                                                                            & Themida, ArXan                                                                                                                             & - Game client might crash because of anti-debugging routines                                                                                                    \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Network-side detection}} & Payload encryption                                                                       & -                                                                                                                                          & \begin{tabular}[c]{@{}l@{}}- High latency, more computing power\\  needed for en/decryption\end{tabular}                                                        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & \begin{tabular}[c]{@{}l@{}}Packet header checking\\ (e.g. TTL, window size)\end{tabular} & -                                                                                                                                          & - High FP rate, heavy analysis cost                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Server-side detection}}  & \begin{tabular}[c]{@{}l@{}}In-game log analysis\\ Data mining\end{tabular}               & AION by NCSoft                                                                                                                             & \begin{tabular}[c]{@{}l@{}}- Low availability\\ - Performance degradation because of client activity analysis\end{tabular}                                      \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                        & Out-game log analysis                                                                    & \begin{tabular}[c]{@{}l@{}}Windows event sequence, geographical location, \\ input patterns from HID (Human Interface Device)\end{tabular} & - Privacy issue                                                                                                                                                 \\ \hline
\end{tabular}
}
\end{table*}







==> paper/cheat-examples-tbl.tex <==
% \begin{table*}[t]
% \centering
% \caption{\hkk{Cheating examples in FPS game}}
% \label{table:cheating_example}
% \begin{tabular}{l|p{7cm}|p{7cm}|}
% \cline{2-3}
%                                              & \textbf{Cheating examples in FPS game}  
%                                              & \textbf{Countermeasure}                                                                         \\ \hline
% \multicolumn{1}{|l|}{\textbf{Application-level}}  & Aimbot, triggerbot, world-hacking, ESP, Twinking, Scriptting, Game element manipulation 
% % & Signature-based, developer's/third-party's security solution, software obfuscation,  Sandboxing 
% \\ \hline
% \multicolumn{1}{|l|}{\textbf{OS-level}}      & Graphical data manipulation, Rapid firing assistance
% % & Verifying (graphic) driver sign                                                                   
% \\ \hline
% \multicolumn{1}{|l|}{\textbf{Network-level}} & Network lag induction, disconnecting 
% % & DDoS mitigation techniques                                                                      
% \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
\begin{tabular}{c|l|}
\cline{2-2}
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\textbf{Cheating examples in FPS games}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Application-level}} & \begin{tabular}[c]{@{}l@{}}Game element manipulation, World-hacking, \\ WSP, Scriptting\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{OS-level}} & \begin{tabular}[c]{@{}l@{}}Aim-bot, Map-hack, Graphical data manipulation, \\  Wall-hack, Rapid firing assistance \end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{Network-level}} & Network lag induction, Disconnecting \\ \hline
\end{tabular}
\caption{Cheating examples in FPS games}
\label{table:cheating_example}
\end{table}
